Preference-grounded Token-level Guidance for Language Model Fine-tuning

Aligning language models (LMs) with preferences is an important problem in natural language generation. A key challenge is that preferences are typically provided at the sequence level while LM training and generation both occur at the token level. There is, therefore, a granularity mismatch between the preference and the LM training losses, which may complicate the learning problem. In this paper, we address this issue by developing an alternate training process, where we iterate between grounding the sequence-level preference into token-level training guidance, and improving the LM with the learned guidance. For guidance learning, we design a framework that extends the pairwise-preference learning in imitation learning to both variable-length LM generation and the utilization of the preference among multiple generations. For LM training, based on the amount of supervised data, we present two minimalist learning objectives that utilize the learned guidance. In experiments, our method performs competitively on two distinct representative LM tasks -- discrete-prompt generation and text summarization.

==> Tex/Applications.tex <==
% \vspace{-10em}
\subsection{Tasks and Setups}\label{sec:appls}
% intro to the two applications (specified notations)
% policy learning in each applications
% reward in each applications

We test our framework on two text-sequence generation tasks with distinct nature:
% how to utilize the learned reward function $r_\phi$ to train the policy LM $\pi_\theta$, by 
\textbf{1)} input-agnostic discrete text-prompt generation for few-shot text-classification (\Secref{sec:app_prompt}),
\textbf{2)} the classical text summarization (\Secref{sec:app_summa}).
Our LM training directly starts from raw pretrained models from HuggingFace  \citep{huggingface2019}, without task-specific supervised pre-training.
Depending on the task-specific LM $\pi_\theta$, our reward function $r_\phi$ can be implemented as either a decoder-only  or an encoder-decoder model.
% , with an additional small MLP projecting the hidden representation into a scalar value.
Similar to prior works \citep[\eg,][]{snell2022offline,menick2022teaching}, given a text sequence $\va$ and an LM input $x$, the causal mask in transformers enables us to get the learned guidance $r_\phi(s_t, a_t)$ at each step of the sequence in parallel.        % $r_\phi(s_t, a_t) = r_\phi((x, a_{< t}), a_t) = r_\phi(x, a_{\leq t})$
Source codes are anonymously \href{https://anonymous.4open.science/r/token_level_reward_learning-5445}{released}.


\subsubsection{Input-agnostic Discrete-prompt Generation} \label{sec:app_prompt}
\myparagraph{Overview.}
In discrete text-prompt generation \citep[\eg,][]{gpt32020,an2022input}, we input a discrete text-prompt $\va$ and an observation sequence $o$ to a large pre-trained Downstream LM $\pi_\dlm(\cdot \given \va, o)$ to directly classify text $o$, without finetuning $\pi_\dlm$.
We follow the classical setting \citep[\eg,][]{schick2020s,rlprompt2022} to perform classification by selecting tokens corresponding to some predefined class labels.
In our input-agnostic setting, the generated prompt is independent of the observation $o$. 
During inference time, only the learned prompts are used and the LM $\pi_\theta$ is discarded.
The initial input $x$ to $\pi_\theta$ is a dummy, and the target $y$ is the class label.
We also adopt the standard few-shot setting \citep{perez2021true}, where both the training and validation sets have $16\, (o, y)$-pairs per class.
With a fixed length $T$, the goal is to find discrete text-prompts $\va = (a_0, \ldots, a_{T-1})$ that have high test accuracy.
We simulate the sequence-level preference by the stepwise metric in \citet{rlprompt2022}, \ie, the higher value the better prompt.
This choice ensures a fair comparison and avoids a potential overfitting --- training and testing the LM on the same evaluation metric ``accuracy''.
Appendix~\ref{sec:details_prompt_tasks} discusses more details about the prompt task.

\myparagraph{LM Training, Implementation, and Datasets.}
Since the prompt-generation task does not assume the availability of supervised data --- the ground-truth prompts, the LM $\pi_\theta$ is trained by the REINFORCE-style update in \Secref{sec:policy_training_without_data} to discover highly-accurate prompts by itself.
% ground-truth
% \myparagraph{Implementation.}
% For the prompt task, 
We implement our framework on the codebase of RLPrompt \citep{rlprompt2022}, and adopt the standard datasets and most hyperparameter setting in it.
The reward training is reconducted every $1000$ steps during the first half of the LM training
and has early stopping.
The reward function is learned with $5$ sampled sequences and the temperature $\beta=2$ in Eq.~\eqref{eq:max_agg}.
The balancing coefficient in Eq.~\eqref{eq:prompt_pol_objective} is $\alpha = 2^{-3}$.
Appendix~\ref{sec:more_abla} discusses the choices of these hyperparameters.
The length of the generated prompts is fixed at $5$.
% Appendix~\ref{sec:prompt_details} provides additional experiment details.
% \myparagraph{Datasets.}
We test on three popular few-shot datasets in prior work \citep[\eg,][]{gao2020making,sun2022black}: the sentiment binary-classification datasets SST-2 \citep{socher2013recursive} and Yelp Polarity \citep{zhang2015character}, and the topic four-way-classification dataset AG News \citep{zhang2015character}.
Additional details on the experiment and the datasets are provided in Appendix~\ref{sec:prompt_details}.




\subsubsection{Text Summarization} \label{sec:app_summa}

\myparagraph{Overview.}
In the summarization task, we follow the standard setting \citep[\eg,][]{t52020,nlpo2022}, where a set of supervised samples is available.
The LM input $x$ is the text to be summarized and the target $y$ is the given summary.
We simulate the sequence-level preference by the classical Meteor score \citep{meteor2005} and report the standard ROUGE scores, to avoid overfitting the evaluation metrics as in the prompt task.


\myparagraph{LM Training, Implementation, and Datasets.}
Since a supervised dataset $\gD$ is available in this task, the LM $\pi_\theta$ can be trained by the weighted-MLE objective in \Secref{sec:policy_training_with_data}.
This objective could be more stable and computationally efficient than REINFORCE-style methods in tasks of long-sequence generation.
% \myparagraph{Implementation and Datasets.}
Due to limited computing resources, unless explicitly mentioned,
we use the standard T5-small model \citep{t52020} for the LM and the reward function.
The reward training is simply $1$ epoch of training on randomly sampled $10\%$ of the training set and is repeated every $0.5$ epochs during the first $2$ epochs of LM training. 
% Each reward training is simply $1$ epoch of training on randomly sampled $10\%$ of the training set.
The reward function is learned with $3$ sampled sequences and again the temperature $\beta=2$ in Eq.~\eqref{eq:max_agg}.
% Appendix~\ref{sec:more_abla} discusses the choices of these parameters.
Additional experiment details are in Appendix~\ref{sec:suma_details}.
We test on the standard setting of two news summary datasets: CNN/DailyMail (CNN/DM) \citep{hermann2015teaching} and XSum \citep{narayan2018don}.



==> Tex/connection_rl.tex <==
\section{Connection with RL-based LM Training}\label{sec:connect_with_rl}

% there has been a long thread in applying RL to NLP, in order to directly optimize discrete metric
There are abundant works in applying RL methods to LM tasks \citep[\eg,][]{stiennon2020learning,ranzato2015sequence,rennie2017self,paulus2017deep,ryang2012framework,rlprompt2022,nlpo2022}, to directly optimize a non-differentiable task metric, such as BLEU \citep{bleu2002}, ROUGE \citep{rouge2004}, or human preference.
% using RL in NLP has the problem of delayed-feedback similar to the hierachy mismatch in our paper
Similar to the preference relations, most of these task metrics are sequence-level, which can suffer the RL-based LM training by the delayed-feedback issue mentioned in \Secref{sec:intro}.
% some paper just ignore this problem, other paper add a KL stabalizer that is unrelated  to the task
Some prior works simply ignore this issue \citep[\eg,][]{ryang2012framework,snell2022offline}. 
Some others add a KL stabilizer less-targeted to the task and metrics, such as a per-token penalty towards a prior distribution \citep[\eg,][]{offlinerldialog2019,sqltext2021,rlprompt2022,nlpo2022}.
% our token-level reward can potentially tackle this problem directly
By grounding the preference among multiple text sequences, our token-level guidance can potentially  tackle the delayed-feedback problem directly and task-specifically.
In the experiments (\Secref{sec:exp}), we compare our approach with strong recent methods that apply RL to LM tasks but under the delayed feedback.

% by the formulation of classification as a contextual bandit problem, our minimalist LM training method can be viewed as RL with $\gamma=0$. [then justify our REINFORCE method and WMLE(by CRR)]

Though not the intention or motivation of our paper, by the formulation of classification as a contextual bandit problem \citep{doublerobustbandit2014}, our \textit{minimalist} LM-training methods can be viewed as RL methods under the myopic but legitimated choice of discount factor $\gamma=0$ \citep{rlintro2018,ddpg2016,ghavamzadeh2015bayesian,bestdice2020}.
Our REINFORCE-style update may then be viewed as standard RL-policy optimization with a max-entropy regularization to capture multiple good behavior-modes, in spirit similar to maximum entropy RL \citep{rlenergypolicy2017,sac2018,sacnew2018}.
More discussions are in Appendix~\ref{sec:rl_reinforce}.
Our reward-weighted MLE objective can be derived as a special case of the standard weighted behavior-cloning method \citep[\eg,][]{crr2020} in  offline-RL  under $\gamma=0$, which may improve upon the vanilla supervised loss (behavior cloning) \citep{crr2020}.
We present the derivation in Appendix~\ref{sec:wmle_offline_rl}.
The discussion here may serve as an extra explanation of our two LM-training losses in \Secref{sec:policy_training}.
Furthermore, \Secref{sec:related_work} provides a literature review on the guiding signals for LM training, especially RL-based methods.
Appendix~\ref{sec:details_rl_nlp} has more detailed discussions on applying RL methods to LM tasks.




==> Tex/method.tex <==
\section{Main Method}\label{sec:main_method}
As discussed in \Secref{sec:intro}, our desiderata is a general framework for learning a token-level reward function that can 
\textbf{(1)} accommodate a more flexible choice of the aggregation function than the classical summation in \Secref{sec:pairwise_pref};
and \textbf{(2)} align with the preference among multiple generated sequences, rather than just pairwise preference in \Secref{sec:pairwise_pref}.

Below we first build our reward-learning framework (\Secref{sec:method_framework}), followed by a discussion on the aggregation functions (\Secref{sec:method_agg_func}).
We then describe applications of the learned reward function in the policy training (\Secref{sec:policy_training}).

\subsection{Reward-Learning Framework} \label{sec:method_framework}
% use a notation for aggregation function 
We have $K\geq 2$ generated sequences $(a^1, \ldots, a^K)$ for the same LM input and target $(x,y)$, with associated generation trajectories $(\tau^1, \ldots, \tau^K)$ and with possibly unequal sequence-lengths $(T^1, \ldots, T^K)$.
Assume that there is a preference ordering among these $K$ sequences.
For description simplicity, let the preference ordering be $a^1 \succ \dots \succ a^K \iff \tau^1 \succ \dots \succ \tau^K$.
We make no assumption on the source of the preference, which can come from human ranking or LM-task-specific evaluation on the full sequences, \eg, $\gR(s^1_{T^1}, y) > \cdots > \gR(s^K_{T^K}, y)$.


\begin{figure*}[t]
\centering
% \vspace{-5mm}
\includegraphics[width=13.5cm]{Tex/fig/reward_seq_gen.PNG}
\captionsetup{font=small}
\caption{Overview of the proposed methods. 
``Gen Token'' refers to the generated token. ``Avg, Sum, Min, Max" refers to the aggregate function. ``Seq Eval" refers to the sequence evaluation.
``Policy LM" is the policy language model. The same model is utilized for both the reward model and the policy language model. We use the distilGPT-2 for the prompt generation and use T5-small for the text summarization.
}
% \vspace{-2em}
\label{fig:pipeline}
\end{figure*}


Denote the chosen aggregation function as $f(\cdot)$, which will be discussed in \Secref{sec:method_agg_func}.
For each generation trajectory $\tau^k = \{(s^k_0, a^k_0), \ldots, (s^k_{T^k-1}, a^k_{T^k-1})\}$, our desired token-level reward-function generates a reward for each step as $\{r_\phi(s^k_t, a^k_t)\}_{t=0}^{T^k-1}$.
With aggregation $f(\cdot)$, a sequence-level evaluation $e_\phi(\tau^k)$ for trajectory $\tau^k$ can be obtained by $e_\phi(\tau^k) = f(\{r_\phi(s^k_t, a^k_t)\}_{t=0}^{T^k-1})$.
Our goal is to train the reward function $r_\phi$ such that the parametrized sequence-level evaluations $\{e_\phi(\tau^k)\}_{k=1}^K$ align with the given preference ordering $\tau^1 \succ \dots \succ \tau^K$.

Under the Plackett-Luce choice model \citep{plackett1975analysis,luce2012individual}, the parametrized sequence evaluations $\{e_\phi(\tau^k)\}_{k=1}^K$ induce a probability distribution over all possible permutations of $\{1, \ldots, K\}$.
We want to maximize the likelihood of the given preference order $\mathrm{ord} = (1,\ldots,K)$, \ie,
\begin{equation} \label{eq:listmle} \textstyle
\resizebox{.91\linewidth}{!}{%
$
     \begin{aligned}
         \min_\phi \gL(\phi) =:& -\log P\br{\mathrm{ord} \given \{e_\phi(\tau^k)\}_{k=1}^K}\,, \text{with} \\
         P\br{\mathrm{ord} \given \{e_\phi(\tau^k)\}_{k=1}^K} =& \prod_{{k=1}}^{K} \cbr{\exp(e_\phi(\tau^k)) \bigg/ \sum_{{i=k}}^{K}\exp(e_\phi(\tau^i))} \,.
     \end{aligned}
$%
}
\end{equation}
When $K=2$ and $f(\cdot)$ denotes \textit{summation}, Eq.~\eqref{eq:listmle} reduces to the classical pairwise-preference loss Eq.~\eqref{eq:original_pref_rew}.
Therefore, our reward-learning loss can be viewed as an extension of the classical pairwise loss.
Our loss Eq.~\eqref{eq:listmle} also extends the ListMLE loss \citep{listmle2008} in the recommender system into the setting of multi-step sequential decision making.

Algo.~\ref{algo:reward_learning} summarizes our reward-learning framework by describing an online-learning routine for training $r_\phi$. 
An offline or hybrid version can be obtain with minor changes.

\begin{algorithm}[H]
% \captionsetup{font=small}
\caption{An online-learning routine for training $r_\phi$. }
\label{algo:reward_learning}
\begin{algorithmic}
\STATE \textbf{Input:} The policy $\pi_\theta$, initialized reward-function $r_\phi$, aggregation function $f(\cdot)$, reward-training steps $M_{\mathrm{rew}}$.
% \STATE
\FOR{$\mathrm{iter} \in \{1, \ldots,M_{\mathrm{rew}}\}$}
\STATE Use $\pi_\theta$ to generate $K$ sequences $(a^k)_{k=1}^K$.
\STATE Get the preference ordering among $(a^k)_{k=1}^K$.
\STATE With $f(\cdot)$, get evaluations $\{e_\phi(\tau^k)\}_{k=1}^K$ from $r_\phi$.
\STATE Optimize $r_\phi$ by Eq.~\eqref{eq:listmle}.
\ENDFOR
\STATE \textbf{Output:} Trained token-level reward-function $r_\phi$. 
\end{algorithmic}
\end{algorithm}


\subsection{Aggregation Function} \label{sec:method_agg_func}
This section discusses some possible choices of the aggregation function $f(\cdot)$, which combines token-level rewards $\{r_\phi(s^k_t, a^k_t)\}_{t=0}^{T^k-1}$ to form a sequence-level evaluation $e_\phi(\tau^k) = f(\{r_\phi(s^k_t, a^k_t)\}_{t=0}^{T^k-1})$ for a trajectory $\tau^k$.

\myparagraph{Summation.} In the classical pairwise-preference loss Eq.~\eqref{eq:original_pref_rew}, $f(\cdot) =\sum (\cdot)$, \ie, $e^{\mathrm{sum}}_\phi(\tau^k) = \sum_{t=0}^{T^k-1}r_\phi(s^k_t, a^k_t)$.

As discussed in \Secref{sec:intro}, when $(T^1, \ldots, T^K)$ are unequal, using \textit{summation} as the aggregation can be confounded by the difference in sequence lengths.
The true ranking, however, may focus more on the generation quality than length in many NLP tasks such as text summarization.
For example, if the token-level rewards are positive, \ie, $r_\phi > 0$, a longer sequence naturally has a higher sum of per-step rewards than a shorter one, which bias $r_\phi$ towards ranking longer sequences higher.
This bias can hinder our reward-learning goal of aligning $\{e_\phi(\tau^k)\}_{k=1}^K$ with the given preference.

To mitigate the effect of unequal sequence lengths in NLP tasks, we consider using the \textit{average}, \textit{soft maximum}, and \textit{soft minimum} as the aggregation function $f(\cdot)$.

\myparagraph{Average.}
We define the average-aggregated sequence-level evaluation $e^{\mathrm{avg}}_\phi(\tau^k)$ for trajectory $\tau^k$ as
\begin{equation} \label{eq:avg_agg}\textstyle
\resizebox{0.91\linewidth}{!}{%
$
e^{\mathrm{avg}}_\phi(\tau^k) = \frac{C}{T^k}\sum_{t=0}^{T^k-1} r_\phi(s^k_t, a^k_t), C = \frac{1}{K} \sum_{k=1}^{K} T^k,
$%
}
\end{equation}
where $C$ is the average length of the $K$ sequences.
Multiplying all $K$ raw average-aggregated rewards by the same average length $C$ does not stain the evaluations by unequal sequence lengths.
It has the benefit of scaling $e^{\mathrm{avg}}_\phi$ to the scale of $e^{\mathrm{sum}}_\phi$, which ensures numerical consistency and reduces hyper-parameter tuning in a modular implementation.

\myparagraph{Soft Maximum and Soft Minimum.}
We define the soft-maximum-aggregated sequence-level evaluation $e^{\max}_\phi(\tau^k)$ for trajectory $\tau^k$ as
\begin{equation}\label{eq:max_agg}\textstyle
e^{\max}_\phi(\tau^k) = C \times \beta \cdot \log \sbr{\sum_{t=0}^{T^k-1} \exp(r_\phi(s^k_t, a^k_t)  / \beta)},
\end{equation}
where $C$ is the average trajectory-length in Eq.~\eqref{eq:avg_agg}, and $\beta$ is the temperature parameter.
Again, multiplying the raw soft maximum by $C$ keeps $e^{\max}_\phi$ to a similar scale as $e^{\mathrm{sum}}_\phi$.
The soft-minimum-aggregated evaluation $e^{\min}_\phi(\tau^k)$ can be obtained by changing $\beta$ to $-\beta$ in Eq.~\eqref{eq:max_agg}.


\subsection{Policy-LM Training} \label{sec:policy_training}
Depending on the data availability, the learned token-level reward function can be applied to policy-LM training in two ways:
\textbf{(1)} a policy-gradient-style update when there is no supervised ``golden'' data (\Secref{sec:policy_training_without_data});
\textbf{(2)} weighted-MLE when there are sufficient supervised data (\Secref{sec:policy_training_with_data}).

Our policy-LM $\pi_\theta$ is a pre-trained LM depending on the concrete task, without task-specific supervised pre-training.
This choice is to keep the algorithm general and consistent in both situations we consider, since task-specific pre-training may not be feasible in the few/zero-shot learning setting.

% alternate between policy learning and reward learning
As shown in Algo.~\ref{algo:reward_learning}, we train the token-level reward $r_\phi$ by sequences sampled from $\pi_\theta$.
Since task-specific pre-training to $\pi_\theta$ is not assumed, over the course of training, $\pi_\theta$ itself can evolve from a less-rewarded distribution to a highly-rewarded one.
To mitigate the impact of this distribution shift, we periodically re-estimate $r_\phi$ during the first half of the policy-learning process, motivated by recent works in model-based RL \citep{mnm2021,wmopo2021,wmbrl2022}.  % without re-initialization, 

\subsubsection{Without Supervised ``golden'' Data} \label{sec:policy_training_without_data}
In the situation where the policy-LM $\pi_\theta$ needs to discover good generations itself, policy-gradient methods can naturally be applied to the training of $\pi_\theta$.
With the learned token-level reward $r_\phi(s_t,a_t)$, we adopt the classical REINFORCE method \citep{reinforce1992} that trains the policy by the gradient
$
\E_{  a_t \sim \pi_\theta(\cdot \given s_t)}[G_\phi^{\pi_{\theta}}(s_t, a_t) \cdot \nabla_{\theta} \log \pi_{\theta}(a_t \given s_t)]
$, % (x,y)\sim \gD,
where $G_\phi^{\pi_{\theta}}(s_t, a_t)$ is the (discounted) accumulated future token-level reward that the policy LM $\pi_\theta$ receives, starting from state $s_t$ and action $a_t$.
When the discount factor $\gamma > 0$, estimating $G_\phi^{\pi_{\theta}}$ requires on-policy Monte-Carlo sampling, which has high variance; or off-policy temporal-difference methods, which require learning an additional value function.
In our preliminary study, we find that both approaches incur additional instability and computational complexity to the training of $\pi_\phi$.
For simplicity, we set the discount factor $\gamma = 0$, and hence $G_\phi^{\pi_{\theta}}(s_t, a_t) = r_\phi(s_t, a_t)$.
\Secref{sec:exp_abla} presents an ablation study of using Monte-Carlo sampling to estimate $G_\phi^{\pi_{\theta}}(s_t, a_t)$ under $\gamma = 1$.
Additionally, since we want multiple generations in typical NLP tasks, instead of only one, we stain the convergence of the REINFORCE method by adding a max-entropy objective.
Therefore, the policy LM $\pi_\theta$ is trained by the gradient 
\begin{equation} \label{eq:prompt_pol_objective} \textstyle
% \resizebox{.91\linewidth}{!}{%
% $
     \begin{aligned}
         & \E_{  a_t \sim \pi_\theta(\cdot \given s_t)}[r_\phi(s_t, a_t) \cdot \nabla_{\theta} \log \pi_{\theta}(a_t \given s_t)]  \\
         & \quad + \alpha \cdot \nabla_\theta \gH(\pi_\theta(\cdot \given s_t)) \,,
     \end{aligned}
% $%
% } % (x,y)\sim \gD,
\end{equation}
where $\gH(\pi_\theta(\cdot \given s_t))$ is the Shannon entropy of $\pi_\theta(\cdot \given s_t)$ and $\alpha$ is a balancing coefficient.



\subsubsection{With Supervised Data} \label{sec:policy_training_with_data}
Assume that a set $\gD = \{(x^{(i)}, y^{(i)})\}_{i=1}^N$ of supervised data is available, we can train the policy LM $\pi_\theta$ by token-level weighted-MLE, where the per-token weight is given by the learned reward-function $r_\phi$.
Our intention is to emphasize the important tokens in the given sequence $y$ and down-weight the unimportant ones.
Specifically, $\pi_\theta$ is trained~by 
\begin{equation} \label{eq:sum_pol_objective} \textstyle
     \begin{aligned}
         & \min_{\theta} -\E_{(x,y) \sim \gD}\sbr{\sum_{t=0}^{|y|-1} w_t \cdot \log \pi_\theta(y_t \given s_t)} \,,  \\
          \text{with } & s_t = (x, y_{< t}) \text{ and } w_t = \frac{r_\phi(s_t, y_t)}{ \sum_{t'=0}^{|y|-1} r_\phi(s_{t'}, y_{t'})}  \,,
     \end{aligned}
\end{equation}
where $|y|$ is the length of $y$ and $w_t$ is the self-normalized token-level reward.
Self-normalization is used to mitigate the variation among samples in $\gD$.

Algo.~\ref{algo:pol_reward_learning} summarizes our policy-reward learning process, with the reward-learning routine specified in Algo.~\ref{algo:reward_learning}.

\begin{algorithm}[H]
% \captionsetup{font=small}
\caption{An alternating policy-reward learning process.}
\label{algo:pol_reward_learning}
\begin{algorithmic}
\STATE \textbf{Input:} The dataset $\gD$, initialized policy $\pi_\theta$, initialized reward function $r_\phi$, policy-training steps $M_{\mathrm{pol}}$, reward-retrain period $M_{\mathrm{re}}$, all reward-training inputs in Algo.~\ref{algo:reward_learning}.
% aggregation function $f(\cdot)$, aggregation function $f(\cdot)$, reward-training steps $M_{\mathrm{rew}}$,
\STATE \textbf{Initialize} $r_\phi$ by Algo.~\ref{algo:reward_learning}.
\FOR{$\mathrm{iter} \in \{1, \ldots,M_{\mathrm{pol}}\}$}
\IF{$\mathrm{iter} \leq M_{\mathrm{pol}} / 2~\mathrm{and}~\mathrm{iter}~\%~M_{\mathrm{re}}$ == 0}
\STATE Re-train $r_\phi$ by Algo.~\ref{algo:reward_learning} without re-intialization.
\ENDIF
\STATE Optimize $\pi_\theta$ by Eq.~\eqref{eq:prompt_pol_objective} or Eq.~\eqref{eq:sum_pol_objective} with $\gD$ and $r_\phi$.
\ENDFOR
\STATE \textbf{Output:} Trained policy-LM $\pi_\theta$. 
\end{algorithmic}
\end{algorithm}

==> Tex/tab/tables_rebuttal.tex <==
\clearpage

\setcounter{table}{0}
\renewcommand{\thetable}{\Alph{table}}

\begin{table}[H]
% \vspace{-1em}
% \captionsetup{font=small}
\caption{
% \small
Average human ratings on CNN/DM summarization under the T5-base LM. 
More details are on the text of \textbf{General Response Q1}.
Summaries are scored on a 5-Point Likert Scale \{1, 2, 3, 4, 5\}, where score 5 is the highest and 1 the lowest.
We bold the best result apart from the ground-truth Reference summary.
} 
% \label{table:longer_prompt}
\centering 
% \vspace{-.7em}
 % \setlength\tabcolsep{15pt}
% \renewcommand{\arraystretch}{1.1}
% \resizebox{\textwidth}{!}{
% \footnotesize
\begin{tabular}{@{}ccccc|c@{}}
\toprule
                     & Supervised & Supervised+PPO & Supervised+NLPO & Ours & Reference \\ \midrule
Average Human Rating & 2.92       & 3.17           & 3.29            & \textbf{3.61} & 3.88      \\ \bottomrule
\end{tabular}
% }
% \vspace{-1.5em}
\end{table}


\begin{table}[H]
% \captionsetup{font=small}
\caption{
% \small
Detailed results on CNN/DM summarization under \textbf{T5-base LM} for \Secref{sec:main_result_suma}, with \textit{BERTScore} results. 
We bold the best result of each metric.
Baseline results are directly cited from RL4LMs \citep{nlpo2022}.
``Env. Reward'' denotes the environmental reward in RL4LMs.
The ``ROUGE-L'' here refers to ``Rouge-LSum'' in RL4LMs and in the Hugging Face interface, which is discussed in details in Appendix~\ref{sec:suma_details}.
We report the mean results of our method over three random seeds.
} 
% \label{table:suma_t5base}
\centering 
% \vspace{-.7em}
 % \setlength\tabcolsep{15pt}
% \renewcommand{\arraystretch}{1.1}
% \resizebox{\textwidth}{!}{
% \footnotesize
\begin{tabular}{@{}llllllll@{}}
\toprule
Algorithm                          & Env. Reward & ROUGE-1      & ROUGE-2      & ROUGE-L  & Meteor & BertScore    \\ \midrule
Lead-3                             &             & 40.1         & 17.5         & 36.3     &   33.3 & 87.4 \\ \midrule
Supervised                         &             & 41.1         & 17.7         & 34.3    &   30.9 &  87.6 \\ \midrule
\multirow{3}{*}{PPO}               & Rouge-1     & 41.0         & 18.2         & 34.9     &  27.6 & 87.6  \\
                                   & Rouge-Avg   & 39.6         & 17.6         & 33.8     &   27.0 & 87.4 \\
                                   & Meteor      & 40.8         & 17.8         & 34.2     &   30.1 & 87.3 \\ \midrule
\multirow{3}{*}{NLPO}              & Rouge-1     & 40.4         & 18.0         & 34.4    &  27.5   & 87.5 \\
                                   & Rouge-Avg   & 40.4         & 17.7         & 34.4    &   27.4 &  87.4 \\
                                   & Meteor      & 40.5         & 18.0         & 34.3     &  29.2  & 87.2 \\ \midrule
\multirow{3}{*}{Supervised + PPO}  & Rouge-1     & 41.7         & 18.9         & 35.8      &  27.8 & 88.2 \\
                                   & Rouge-Avg   & 42.5         & 19.4         & 36.3    &   29.6  & 88.2 \\
                                   & Meteor      & 42.6         & 19.4         & 36.1    &   31.6  & 88.0 \\ \midrule
\multirow{3}{*}{Supervised + NLPO} & Rouge-1     & 42.1         & 19.3         & 36.1   &   28.7  &  88.2 \\
                                   & Rouge-Avg   & 42.4         & 19.3         & 36.3   &    29.5 &  88.2 \\
                                   & Meteor      & 42.9         & 19.4         & 36.1   &    31.9 &  88.0 \\ \midrule
Ours    (AVG)                           &             & \textbf{43.09}  & \textbf{20.17}  & \textbf{39.99}  & \textbf{35.23} & \textbf{89.61}  \\
Ours  (SUM)   &     & 42.86   & 19.92   &  39.76   &  34.74 & 89.24  \\
Ours  (MIN)    &    & 42.92   &  20.01  & 39.84   &  34.88  &  89.33 \\
Ours  (MAX)     &   & 42.38   &  19.49  & 39.34   &  34.13  & 89.09 \\  
\bottomrule
\end{tabular}
% }
% \vspace{-1.5em}
\end{table}






==> Tex/tab/use_r_vs_q.tex <==
\begin{table}[tb]
\small
\def\arraystretch{1.3}
\setlength\tabcolsep{23pt}
 
\captionsetup{font=small}
\caption{
Results on changing $r_\phi$ to $G_\phi^{\pi_{\theta}}$ in Eqs.~\eqref{eq:prompt_pol_objective} and \eqref{eq:sum_pol_objective}.
Number reporting and abbreviations follow Tables~\ref{table:prompt_main} and \ref{table:suma_main}.
} 
\label{table:use_r_vs_q}
\centering 
% \renewcommand{\arraystretch}{1.1}
% \resizebox{\textwidth}{!}{
\vspace{-.8em}
\begin{tabular}{@{}l|ll@{}}
\toprule
\small{SST-2}    & Use $r_\phi$ & Use $G_\phi^{\pi_{\theta}}$ \\ \midrule
Accuracy & 92.60 {\scriptsize (1.7)}   & 84.40 {\scriptsize (4.3)}                  \\ \midrule\midrule
CNN/DM   & Use $r_\phi$ & Use $G_\phi^{\pi_{\theta}}$ \\ \midrule
ROUGE-1  & 40.87 {\scriptsize (0.02)} & 40.26 {\scriptsize (0.08)}                \\
ROUGE-2  & 18.77 {\scriptsize (0.02)} & 18.04 {\scriptsize (0.07)}                \\
ROUGE-L  & 38.10 {\scriptsize (0.02)}  & 37.59 {\scriptsize (0.08)}                \\ \bottomrule
\end{tabular}
% }
% \vspace{-.1em}
\end{table}
